DBL: Efficient Reachability Queries on Dynamic Graphs (Complete Version)

Reachability query is a fundamental problem on graphs, which has been extensively studied in academia and industry. Since graphs are subject to frequent updates in many applications, it is essential to support efficient graph updates while offering good performance in reachability queries. Existing solutions compress the original graph with the Directed Acyclic Graph (DAG) and propose efficient query processing and index update techniques. However, they focus on optimizing the scenarios where the Strong Connected Components(SCCs) remain unchanged and have overlooked the prohibitively high cost of the DAG maintenance when SCCs are updated. In this paper, we propose DBL, an efficient DAG-free index to support the reachability query on dynamic graphs with insertion-only updates. DBL builds on two complementary indexes: Dynamic Landmark (DL) label and Bidirectional Leaf (BL) label. The former leverages landmark nodes to quickly determine reachable pairs whereas the latter prunes unreachable pairs by indexing the leaf nodes in the graph. We evaluate DBL against the state-of-the-art approaches on dynamic reachability index with extensive experiments on real-world datasets. The results have demonstrated that DBL achieves orders of magnitude speedup in terms of index update, while still producing competitive query efficiency.

==> secs/Response.tex <==
\section*{\centering{Response to Reviewers' Comments}}


We thank the reviewers for the insightful comments. We have revised the manuscript and indicated the changes in blue. In the following, we provide detailed responses to each reviewer. We will use RXWY to refer to the weak point Y raised by reviewer X. Similarly, RXDY refers to the detailed evaluation Y provided by reviewer X.


\subsection*{Response to Reviewer 1}

\begin{itemize}
\item \textbf{R1W1:}Though the idea of landmark and leaf labels are catchy, the usage of the labels are not explored in an exhaustive manner.
\item \textbf{R1D1:}The usage of DL and BL in Algorithm 1 is leading towards a high query processing time. It might be useful to explore more about the profiling the checking part (DL\_Intersec and BL\_contain) and the BFS part afterwards. Based on the profiling and given network data, a more efficient query processing algorithm can be built.
\end{itemize}

\textbf{Response:}DBL's query processing include two parts: Label query and pruned BFS query. Generally, DL and BL label could answer nearly 99 percent of the query. But the BFS process is much more time consuming. We have profiling the query process and the result is shown in Table~\ref{tab:query-profiling}.



\begin{itemize}
\item \textbf{R1D2:}Section 4: second para \--- Why is the space complexity $O(\mid L\mid)$, should not it be $O(n\mid L\mid)$?
\end{itemize}

\textbf{Response:}We agree that the space complexity should be $O(n\mid L\mid)$. The error have been corrected in the paper.

\begin{itemize}
\item \textbf{R1D3:}"... the optimal landmark selection can be reduced to the maximum set cover problem" --- This statement is conceptually wrong to prove NP-hardness. The correct way is the following: A known NP-hard problem has to be reduced to the problem in hand (in this case, the landmark selection problem).
\end{itemize}

\textbf{Response:}The statement have been modified in blue.


\begin{itemize}
    \item \textbf{R1D4:}How do you choose BL labels? It needs to be discussed. The quality will depend on the nodes in BL (given that only k' is being chosen).//Ñ¡µãÊµÑé
\end{itemize}


\textbf{Response:}BL label selection have been discussed in the appendix. In theory, we could choose all the nodes that $|Pre(v)|*|Suc(v)|<r$ as the label node. But our experiment(figure 15) have shown that more label node will not make the BL label more efficiency(more label node bring a higher hash collision rates), so we use all the leaf nodes that $|Pre(v)|*|Suc(v)|=0$ as the BL label node in the main body of the paper.


\begin{itemize}
\item \textbf{R1D5:}What about node insertions and deletions in dynamic graphs? It would be good to have a discussion about them.
\end{itemize}

\textbf{Response:} In fact, every node operation is just consist of a set of edge operation. For example, when insert node $u$, we need to update $u's$ BL and DL label. In DBL manner, we will insert all the edges that related to the inserted node. Node deletion is handled in similar manner. When delete node $u$, all the related edges(adjacent edge) will be deleted. Thus, a node operation is transformed into an edge operation. We have modified section~\ref{sec:discussion} to discuss the process.



\begin{itemize}
\item \textbf{R1W2:}The experimental results are limited and could be improved.
\item \textbf{R1D6:}Section 6.2: The parameters in DBL are not being evaluated in systematic manner. As the indexing is just a heuristic, it is expected to have an extensive evaluation on different types of graphs.//¼ÓÍ¼
\item \textbf{R1D7:}Section 6.2: There are claims about a few landmark nodes covering a significant amount of reachability information. First, this kind of claims are not verified on several datasets. Second, it depends on the quality of chosen landmark set. Again the algorithm (in this paper) that chooses this set is also based on a heuristic. So, it expected to have the evaluation about this heuristic.
\end{itemize}



\textbf{Response:}The claim in section 6.2 is not quite appropriate. \textcolor{blue}{It has been modified to clarify the claim.} In fact, we have stated that the DL label will degrade to plain BFS when the underlying graph is poorly connected(second page, coloring in blue). Landmark label will be efficiency when the graph is of high connectivity such as social network. If the graph is sparse with low connectivity, DL label will get a severe performance degrade as the landmark node will cover little reachable information in this scenario.

Landmark selection is a problem that have been well studied. As our landmark selection is degree based, it have been proved in \cite{akiba2013fast}\cite{potamias2009fast} that degree-based landmark selection is efficiency. We have cited the paper to support our claim. The evaluation of the landmark selection will be omit in our paper.




\begin{itemize}

\item \textbf{R1D8:}Section 6.3: The loss in query time needs be reported in numbers. A solid discussion of the set of criterion (regarding the graph structure) that dominates the query time and update time would improve the paper.

\end{itemize}

\textbf{Response:}\textcolor{blue}{ The query cost have been shown in numbers in Table 4. We have modified section 6.3 to discuss the factors that influence the query and update performance of DBL.}



\begin{itemize}
\item \textbf{R1D9:}Section 6.4:The comparison with the baseline needs to be improved. The baseline (IP) is being parallelized in a naive way. It should be improved (similar to the algorithms in the paper) before comparison.
\end{itemize}

\textbf{Response:}\textcolor{blue}{We have improved the parallel efficiency of \ipp. As \ip is a \dfs based method, its query performance will get a limited improve from parallel process. Please refer to Table~\ref{tab:gpus} to get the detail.}



\begin{itemize}
\item \textbf{R1W3:}The writing could be more polished. The algorithms are unnecessarily long and repetitive.

\item \textbf{R1D10:}The algorithms are written in a lazy manner, they are unnecessarily long and repetitive.

\item \textbf{R1D11:}There are many minor mistakes in writing. It will be good if the authors take a pass to remove them.
\end{itemize}

\textbf{Response:}\textcolor{blue}{xxxxxxxxxxxxxxxxxxxxxxxxxxxxx}




\subsection*{Response to Reviewer 2}

\begin{itemize}
\item \textbf{R2W1:}Some statements are not clarified.
\item \textbf{R2D1:}In Page 5, it is better to prove the NP-hardness of landmark selection problem. In Section 4.1, the choice of update method 1) or 2) should be clarified.
\end{itemize}


\textbf{Response:}The NP-hardness of the landmark selection have been proved by \cite{potamias2009fast}. The author reduce the vertex cover problem to the landmark selection scenario. We have cited their work to support our statement. For the update process in section~\ref{sec:lan:insert}, it has been clarified that the first scenario is chosen as our update method. All the modification have been colored blue.



\begin{itemize}
\item \textbf{R2W2:} To better support index update, it sacrifices query efficiency (See D2).
\item \textbf{R2D2:}The proposed approach uses much larger indices and it sacrifices the query time for more efficient update time, as shown in Table 3, Figures 11 and 12.
\end{itemize}



\textbf{Response:}There is a big difference between DBL and the other methods -- DBL works on original graph. As both IP and TOL indexing on DAG which is equivalent in reachability but much smaller in scale, it's natural that they will have smaller index size.

DBL does get a little slower query speed than the other methods. This is because DBL is focus on the update process. Most of the state-of-the-art methods could handle one million query in tens of microsecond. However, the update process is three or four magnitude slower than query. Actually,  update is quite common in real life graph such as social network. Twitter for example, establish a new followship is a normal and frequent operation. We want to argue that, in the frequent update dynamic graph, query speed is not a bottleneck but update is. Thus, sacrifices a little query speed to get an improved update process is reasonable.




\begin{itemize}
\item \textbf{R2W3:}The setting for query processing time is not clear.
\item \textbf{R2D3:}For the query performance in Table 4, it is not clear whether the time is a sum of edge insertions, deletions and query time costs. Besides, please explain why TOL is not compared in Table 4.
\end{itemize}



\textbf{Response:}Table~\ref{tab:gpus} shows the query cost without update. Also, we have modified Table 4 to show TOL's query performance.




\begin{itemize}
\item \textbf{R2W4:}Lack of some related experiments.
\item \textbf{R2D4:} Although the experiments vary the size of DL and BL labels, it is still interesting to examine which set of landmarks lead to better performance, e.g., the high centrality nodes, or the high $|Pre()|+|Suc()|$ nodes. This also arises in the choice of leaf nodes. Currently, it is not clear what the chosen leaf nodes exactly are.
\end{itemize}

\textbf{Response:}The discussion of label node selection is put in appendix. For DL label, we order the vertex with the value of $M(v) = |Pre(v)| * |Suc(v)|$, e.g., the vertices with a larger M value will be selected as landmark node. In fact, it is a degree based method, which have been proved efficiency in \cite{akiba2013fast}\cite{potamias2009fast}. For BL label, figure 15 have shown that selecting more label node will not lead to a better query performance. Thus we choose all the leaf nodes(either the in-degree is zero or the out-degree is zero) as the label node. Less label node will decrease the hash collision rate, thus, provide a better query performance. On the other hand, constructing BL label from leaf node could guarantee that all the vertex in the graph are covered by BL label.


\begin{itemize}

\item \textbf{R2D5:}In Figures 11 and 12, the proposed DBL sometimes has a larger update time for both edge insertion and deletion, e.g., on BerkStan and Twitter. Please show the reason.

\end{itemize}




\textbf{Response:} In Figure~\ref{fig:subfig1} and Figure~\ref{fig:subfig2}, DBL shows a bad performance on BerkStan and Twitter. The main reason is that their query speed is relatively slow. For most of the dataset, \sol label could directly answer nearly 99 percent of the query. However, the number is 94.06 percent for BerkStan and 96.7 percent for Twitter. The unsatisfactory label performance will also lower the pruning capability in BFS query process which will impose extra overheads in query.

\sol's update is a label-based process. The update will be early terminated when the visited vertices' label is unaffected by the edge insertion/deletion. Therefor, it's common that the label's inefficiency will slower the update process.

We also want to emphasize, the update process in \tol and \ip is incomplete. As both of them only works on DAG, they should keep the graph as a DAG if the update process destroy the structure. However, their update process is special designed to avoid the DAG maintaining. Thus, the compare in Figure~\ref{fig:subfig1} and Figure~\ref{fig:subfig2} is in fact unfair for \sol as their method exclude the DAG maintaining overheads.





\subsection*{Response to Reviewer 3}


\begin{itemize}
\item \textbf{R3W1:}The updates in the experiments are synthetic in nature. Thus, the following is not clear: In real-world dynamic graphs setting, how often the strongly connected components (SCC) get updated? Even if the SCCs get updated, and one follows the existing methods [28, 34], how much the error would be? In other words, the motivation of this paper need to be justified with real-world statistics and real-world graph updates.
 \item \textbf{R3W4:}In order to fairly compare DBL with other state-of-the-art methods, the whole experiments do not consider the scenario of updating strongly connected components, but this often occurs in real-world datasets. In fact, this is one of the motivation in their paper.
\item \textbf{R3D4:}Since one main contribution of this paper is that DBL could work even when strongly connected components are changed, it could be better to add relevant experiments. As there is no existing method that directly deals with it, please provide comparisons based on the following: (1) how much query time it would take for a naive bidirectional BFS. (2) If one follows existing methods [28, 34], clearly they cannot deal with such updates. However, how much error their indexes would incur for such updates?
\item \textbf{R3D5:}The updates in the experiments are synthetic in nature. (1) To better motivate the problem, please provide the following statistics: In real-world dynamic graphs setting, how often the strongly connected components (SCC) get updated? Even if the SCCs get updated, and one follows the existing methods [28, 34], how much the error would be? (2) Also add some experimental results with real-world graph updates. Several dynamic and stream graphs can be found in: https://snap.stanford.edu/data/index.html\#temporal and (http://konect. uni-koblenz.de/ networks/

\end{itemize}

\textbf{Response:}\textcolor{blue}{We have added the bidirectional BFS query time in section xxxxxxxxx.}

In fact, both IP and TOL have clarify that they could follow the \dagg maintaining method proposed by \cite{yildirim2013dagger}, but in order to avoid the \dagg maintaining process, their experiment are special designed. It means that, the \dagg maintaining overheads are exclude from their program. DBL is different as it is a work based on the original graph, the \dagg-free feature means that we don't have any \dagg related overheads. Thus, the update experiment in the paper is unfair for \sol.

Clearly, both IP and TOL cannot deal with \dagg-affected updates. TOL for example, its index is based on a special order of the vertices, however, the order is constructed based on topological order. It could be seen from its update algorithm that the update process is also topological order relied. Thus, if the insertion/deletion generate new \scc in the graph, the update process can not go on as it needs topological order of the graph. Similarly, both the construction and update of IP are heavily relied on the topological order. The update algorithm needs topological order to progress the process. Therefor, if we don't maintaining the \dagg, IP and TOL can't go on update processing. So we cannot compute the error rate without \dagg maintaining.

\textcolor{blue}{For real world graph, ...............}



\begin{itemize}
\item \textbf{R3W2:}(i) The space and time complexity of the following need to be discussed clearly and formally: (1) Index building, (2) Index updating, and (3) Query processing. For index updating, both deletion and insertion need to be considered for the complexity analysis.(ii) Moreover, in the worst case, it seems to me that all of these can end up being more expensive BFS in the entire graph. Thus, it needs to be discussed more formally what are the best cases (in terms of graph structure, query nodes, landmark selection, etc.), and what are worst cases? What are average cases (amortized analysis)?(iii) Over time, the landmark nodes themselves can change. Similarly, with the addition/ deletion of edges, zero-in or zero-out degree nodes also change. How these are taken care of?
\item \textbf{R3D6:}(1) Formally discuss the space and time complexity of the following: (a) Index building, (b) Index updating, and (c) Query processing. For index updating, both deletion and insertion need to be considered for the complexity analysis.(2) In the worst case, it seems to me that all of these can end up being more expensive BFS in the entire graph. Thus, it needs to be discussed formally what the best cases are (in terms of graph structure, query nodes, landmark selection, etc.), and what are the worst cases? What are average cases -- amortized analysis could be useful.(3) Over time, the landmark nodes themselves can change. Similarly, with the addition/ deletion of edges, zero-in or zero-out degree nodes also change. How these are taken care of?


\end{itemize}


\textbf{Response:}\textcolor{blue}{XXXXXXXXXXXXXXXXXXXXXXXX}


\begin{itemize}
\item \textbf{R3W3:}The paper presents two rules (DL and BL labels) for finding unreachable node pairs using dynamic landmark labels. However, experiments do not evaluate the effectiveness of each rule separately.
\item \textbf{R3D3:}Experiments should be added to evaluate the effectiveness for each rule (DL and BL labels) separately.
\end{itemize}



\textbf{Response:}Figure 9 and figure 10 shows the effectiveness of the DL and BL label separately. When varying the DL label size we keep the BL label size 64 bit, and vice versa. Figure 9 shows the query time varying with the label length. Figure 10 shows the BFS ratio in query and the average visited vertices with the varying of label length.




\begin{itemize}
\item \textbf{R3W5:}Index building time and memory usage were not compared against existing methods (neither mentioned). Only index updating time and query times are presented.
\item \textbf{R3D7:}Please provide and compare (with [28, 34]) Index building time and memory usage in the experimental results.
\end{itemize}


\textbf{Response:}\textcolor{blue}{Index construction time have been added in section~\ref{index-construction}. Memory xxxxxxxxxxxxx}



\begin{itemize}
\item \textbf{R3W6:}Some experimental results lack proper analyses, for example,(i) why is the query processing time of DBL-G much longer than that of IP-P on the dataset BerkStan and Twitter (In Table 4)?(ii) The way it is currently presented, in Figure-11, over Wiki, BerkStan, and Twitter, the proposed DBL is not the best method. Similarly, in Figure-12, over Web, Pokec, BerkStan, and Reddit, the proposed DBL is not the best method. This primarily happens due to higher query time for DBL over the entire graph (as opposed to [28, 34] working over the DAG). However, this also brings the question if query time is less important (i.e., in what context, it is preferred to have lesser index updating time, at the cost of higher query time)? Such issues need to be well-justified.
\item \textbf{R3D9:}Please add more analyses and explanations in Sec-6, some key points are missing. For example, (1) it is not clear that what the Y-axis in Figure 13 refers to.In particular, "time" on Y-axis need to be clarified as query time, index building time, or index updating time. (2) Why is the query processing time of DBL-G much longer than that of IP-P on the dataset BerkStan and Twitter (in Table 4)?(3) The way it is currently presented, in Figure-11, over Wiki, BerkStan, and Twitter, the proposed DBL is not the best method. Similarly, in Figure-12, over Web, Pokec, BerkStan, and Reddit, the proposed DBL is not the best method. This primarily happens due to higher query time for DBL over the entire graph (as opposed to [28, 34] working over the DAG). However, this also brings the question if query time is less important (i.e., in what context, it is preferred to have lesser index updating time, at the cost of higher query time)? Such issues need to be well-justified.

\end{itemize}


\textbf{Response:}\textcolor{blue}{The Y-axis in figure 13 is query time. We have modified the figure to clarify.}

From figure 11 and 12 we could discover that DBL is not the best method for some dateset. There are two reasons: First, the SCC maintaining overheads are omitted for TOL and IP as they can't handle SCC maintaining process. Therefore, it is actually an unfair compare for DBL as we don't have the overheads. Second, the label answer ratio is relatively low for the dataset. As we test the DBL label efficiency, DL and BL label could directly answer nearly 99 percent of the queries for most of the dataset. However, for BerkStan dataset, the ratio is 94.06 percent and 96.7 percent, which means that much more BFS is needed to answer the query. Furthermore, the inefficiency of the label lead to an inefficiency pruning BFS process which will impose more overheads on query.


It could be seen from table 4 that the DBL-G method is much slower than IP-P in some dataset. This is because that the pruned BFS process on GPU will get little speed up. As we use label to prune the BFS process, the data in each BFS layer is relatively small. Thus GPU can get little speed up in BFS process. For IP-P, different \dfs process are allocated to different threads. Therefor, it is natural that IP-P will perform better than DBL-G in heavily traversal-relied dataset such as BerkStan.


DBL does have a little longer query time than TOL and IP. In fact, DBL is based on dynamic graph which is quite common in real life such as social network. Facebook or Twitter for example, it is very common to establish a friendship(or followship) as a new edge from one person to the other. Existing state-of-the-art method is very efficiency in query whereas get some disadvantages in update. There is a large gap between the query speed and update speed.  One million query could be answered in tens of microseconds but the same scale update will be three or four magnitude slower. We want to argue that for some dynamic graph the query speed is not a bottleneck but update is. Hence, it is reasonable to accelerate the update process at the cost of a little query speed.





\begin{itemize}
\item \textbf{R3D8:}(1) In Sec-3, it is mentioned that landmarks are selected as nodes with high centrality, similarly for BL with low centrality. Please clarify and justify what kind of centrality is being referred to (e.g., degree centrality, between-ness centrality). (2) Moreover, it is stated in Sec-4 that $|Pre(v)|*|Suc(v)|$ is a good measure for centrality. This need to be justified with experimental evidences.
\end{itemize}


\textbf{Response:}\textcolor{blue}{In the paper, we have claimed that the landmark selection is centrality based. It is a little misleading. So we will adopt degree to elaborate the landmark selection.}

Landmark selection is a problem that have been studied for years. Generally, there is three strategies which based on random selection, degree based selection and centrality based selection. It have been proved that random selection will lead to bad performance. In section 4, we propose to use $M(v)=|Pre(v)|*|Suc(v)|$ to rank the landmark nodes. Actually, this is a degree-based method for directed graph. It have been proved in \cite{akiba2013fast}\cite{potamias2009fast} that degree-based landmark selection is a good method and get a suboptimal performance. Most important is that it avoid the complex centrality computation. Although most of the landmark selection method are discussed based on undirected graph, it is natural to extend for directed graph. For undirected graph, landmark nodes are selected according to degree. Because a high degree indicate that the vertex are more likely to be on the key position. Directed graph is different in that there is in-degree and out-degree separately. Only use in-degree or out-degree to measure the importance of the vertex is improper. Thus, for directed graph the product of the in-degree and out-degree is a good replacement for the degree in undirected graph. It could also avoid the selecting of leaf node that either in-degree or out-degree is zero.

We have cite the paper \cite{akiba2013fast}\cite{potamias2009fast} to support our statement, thus we will omit the related proof in our paper.







\begin{itemize}
\item \textbf{R3D10:}(1) How 1 million queries are generated? It needs to be discussed what happens in terms of query time based on the distance distribution between query nodes (e.g., 2-hops away, 4-hops away, 6-hops away, 8-hops away, not reachable). (2) Similarly, in case of synthetic updates, it needs to be discussed if the inserted edges connect two nodes that are 2-hops away, 4-hops away, 6-hops away, 8-hops away, not reachable in the original graph, etc.
\end{itemize}



\textbf{Response:} All the query is generated in random manner. \textcolor{blue}{xxxxxxxxxxxxxxxxxx}



\begin{itemize}
\item \textbf{R3D11:}In Sec-5.1, the paper mentions that since DL labels covers only partial reachability information, this may lead to redundant BFS in Algorithm 4. Actually, this may also happen in Algorithm 2, so it needs to be mentioned in the content for explaining Algorithm 2.
\end{itemize}

\textbf{Response:}Thanks for your comments. We have revised the corresponding section to explain Algorithm 2.



\subsection*{Response to Meta-Reviewer}

\begin{itemize}
\item \textbf{Comment} The reviewers are in agreement that this is a strong paper, but needs to undergo a revision to address quite a few clarification issues and shortcomings of experimental evaluation.
\end{itemize}

\textbf{Response:} Thanks for your comment. We have try our best to address all the reviews. All the modifications are colored blue in the paper.





==> secs/dynamic.tex <==
\section{Dynamic Graph}\label{sec:dg}
In this section we will discuss how to maintain the labels we proposed over dynamic graph. The dynamic graph operation include vertex insertion/deletion and edge insertion/deletion. The vertex insertion/deletion usually consist of one or more edge insertion/deletion, so we will just handle edge insertion/deletion in our work. As we have discussed in preceding section, if we apply 2-Hop method mechanically in dynamic graph, the index size will explode as we insert edges, on the other hand, because 2-Hop label is a Label-only method that have to maintain the index that completely cover all the reachability information, the edge insertion/deletion will usually influence a lot of nodes in source node's \bfs flooding area. As a consequence, the dynamic insertion/deletion process will be both time consuming and space consuming. TOL\cite{zhu2014reachability} is a state-of-the-art reachability index that base on 2-Hop label. It's special order limitation on index could limit the index size growth speed, but still, a lot of nodes that influenced by the insertion/deltion will be searched and the label will be update. Further more, order maintaining process also cause extra overhead.

The main reason for all the shortcoming of 2-Hop label in dynamic graph is that 2-Hop index have too much label node. Again, it is because 2-Hop label is a Label-only method that its label need to completely cover all the reachability information. In fact, all the shortcoming is the overhead of maintaining the completeness of 2-Hop label.


We propose \dl method to handle positive query in dense graphs. It's based on an observation that in dense graph only a few hub node could cover most of the reachable information. In our experiment with some cases like social network, the 2-Hop form label could cover as much as 80 percent reachability information(the number of 1 in transitive closure) with just one label node. \dl method dramatically decrease the number of label node which lead to a significant speed promotion in dynamic graph label maintaining. The limited number of label node will give an upper bound to the index size. For a graph with x label nodes, the upper bound of the index size will be $n*x*2$ where n is the number of vertices in graph. So the \dl index will not explode significantly when we insert edges. Also, the limitation of the label node will lead to an early termination of \bfs process which is a really important component in query. It is obvious that DL index is a specific and targeted method toward the shortcoming of dynamic 2-Hop label.


\bl is a complementary component to \dl label. Due to the hash operation in index construction, the \bl label is good at handling sparse graph. When there are really a lot of insertion operation in graph, the efficiency of \bl label will degrade as the label(in hash set manner) turns to be "full". Same to the \dl label, the update of the \bl label is also benefit from the early terminate of the \bfs process. It is based on an observation that if there exist an edge (u,v) in the graph, the $BL_{in}(u)$ is a subset of  $BL_{in}(v)$ and the $BL_{out}(u)$ is a superset of $BL_{out}(v)$. If we construct \dl label without pruning, the observation should also be applicative to \dl label. Fortunately, the pruned construction process in \dl label will not affect the correctness of \dl's early terminate in edge insertion or deletion.



Quite different from existing work\cite{wei2018reachability} which use several different label to accelerate the query process. The maintaining operation of \dl index and \bl index is consistent which means that we don't need to do label update respectively. When we update \dl and \bl index in dynamic graph, the edge insertion will incur a series of set union operation and the edge deletion will incur computing on set difference.


%
%\begin{algorithm}[ht]
%\caption{Label update for edge insertion}
%\begin{algorithmic}[1]
%\REQUIRE
%Graph G(V,E), Reversed Graph G'(V,E'), \dl index, \bl index, Inserted edge (u,v)
%\ENSURE
%Updated index
%\IF{ $DL_{out}(u) \cap DL_{in}(v)$ }
%\STATE break
%\ENDIF
%\STATE //Do pruned \bfs from v in G(V,E)
%\WHILE{\bfs queue is not empty}
%\FOR{node p that \bfs visited}
%\IF{ $DL_{in}(u) \not\subseteq  DL_{in}(p)$ \newline and $BL_{in}(u) \not\subseteq BL_{in}(p)$ }
%\STATE $DL_{in}(p) |= DL_{in}(u)$
%\STATE $BL_{in}(p) |= BL_{in}(u)$
%\STATE Enqueue p
%\ENDIF
%\ENDFOR
%\ENDWHILE
%\STATE //Do pruned \bfs from u in G'(V,E')
%\WHILE{\bfs queue is not empty}
%\FOR{node q that \bfs visited }
%\IF{$BL_{in}(u) \not\subseteq BL_{in}(q)$}
%\STATE $BL_{out}(q) |= BL_{out}(u)$
%\STATE Enqueue q
%\ENDIF
%\ENDFOR
%\ENDWHILE
%\end{algorithmic}
%\end{algorithm}




\subsection{Edge Insertion}
%\todo{It is better to have some theorems stating the correctness of the index updates!}


We show the label update for edge insertion in Algorithm 4. We have describe the \bl and \dl label in preceding section. \bl index is a 2-Hop form method that the label node is an intermediate of the vertices in graph. As the inserted edge will add extra connectivity to the graph, the affected nodes are in the \bfs flooding area of the inserted edge in both direction, but in fact, we can either update the \dl "in" label in forward direction or "out" label in backward direction as the update operation is equivalent. But the \bl label update will be a bidirectional process as \bl label are constructed bidirectional. With the insertion of edge (u,v), the nodes in v's forward \bfs area will be reachable by all the zero in-degree nodes that could reach u, symmetrically, all the zero out-degree nodes that v could reach will be now reachable by all the nodes that could reach u. Therefore, only set union operation will be needed in our edge insertion update. As both our \bl and \dl label are maintained in a bit set form, we use an "or" operation to do set union. When we get the inserted edge (u,v), we will first detect whether the node v are reachable by node u before the edge insertion (line 1-3), if v is reachable by u, it is certain that the newly inserted edge will not incur label update because the newly inserted edge will not add any extra connectivity. If v is unreachable by u before insertion, we will update label in forward direction and both \dl label and \bl label are updated. Node v's label will be updated and then \bfs from node v will be performed in forward direction (line 5-13). The most important reason for why our method get a faster update speed is that our approach is efficiency in pruning. The update rely on a pruned \bfs in which we will only enqueue nodes that the label will be affected by the edge insertion. For an edge insertion (u,v), taking the forward update process as an example, when our \bfs update process visit node p and the $BL_{in}(u)$ is a subset of $BL_{in}(p)$ which means the set union operation will not affect $BL_{in}(p)$, it is certain that node p will not need to enqueue as all the $BL_{in}$ of its descendent is a superset of $BL_{in}(p)$, all the descendent of node p will be pruned from the forward \bfs process. The update of $BL_{out}$ in backward direction works in exactly same manner. The pruned \bfs for \dl label is in similar way. Although the construction of \dl label is based on a pruned \bfs which is different from \bl's completely \bfs, the pruning update process still guarantee the correctness of the updated label as \dl is not a label-only method, we just need to keep it right without all reachability information fully covered. Therefor, although we insert edge (u,v) and update the \dl label, the \dl label will not guarantee to give a positive answer when we query whether node v is reachable by u.







%\begin{algorithm}[ht]
%\caption{Label update for edge deletion}
%\begin{algorithmic}[1]
%\REQUIRE
%Graph G(V,E), Reversed Graph G'(V,E'), \dl index, \bl index, Deleted edge (u,v)
%\ENSURE
%Updated index
%\STATE Initialise $BL\_Ds_{in}(v) = BL_{in}(u)$ \newline and $DL\_Ds_{in}(v) = DL\_Ds_{in}(u)$
%\FORALL{p in \emph{Pre(v)}}
%\STATE $BL\_Ds_{in}(v) = BL\_Ds_{in}(v) - BL_{in}(p)$
%\STATE $DL\_Ds_{in}(v) = DL\_Ds_{in}(v) - DL_{in}(p)$
%\ENDFOR
%\IF{ $BL\_Ds_{in}(v) \neq \emptyset$ or $DL\_Ds_{in}(v) \neq \emptyset$}
%\STATE $BL_{in}(v) = BL_{in}(v) - BL\_Ds_{in}(v)$
%\STATE $DL_{in}(v) = DL_{in}(v) - DL\_Ds_{in}(v)$
%\STATE //Forward direction update, do \bfs from v
%\STATE Enqueue node v to Queue
%\STATE Enqueue $BL\_Ds_{in}(v)$ to BL\_Ds\_Queue
%\STATE Enqueue $DL\_Ds_{in}(v)$ to DL\_Ds\_Queue
%\WHILE{Queue is not empty}
%\FOR{node p in Queue}
%\STATE Dequeue p
%\FOR{node x in \emph{Suc(p)}}
%%\STATE //Get $BL\_Ds_{in}(p)$ from $BL\_Ds\_Queue$
%\STATE $BL\_Ds_{in}(x) = BL\_Ds_{in}(p)$
%%\STATE //Get $DL\_Ds_{in}(p$) from $DL\_Ds\_Queue$
%\STATE $DL\_Ds_{in}(x) = DL\_Ds_{in}(p)$
%\STATE //Compute the $Ds_{in}$ set for x
%\FOR{node y in \emph{Pre(x)}}
%\STATE $BL\_Ds_{in}(x) = BL\_Ds_{in}(x) - BL_{in}(y)$
%\STATE $DL\_Ds_{in}(x) = DL\_Ds_{in}(x) - DL_{in}(y)$
%\ENDFOR
%\IF{$BL\_Ds_{in}(x) \neq \emptyset$ or $DL\_Ds_{in}(x) \neq \emptyset$}
%\STATE $BL_{in}(x) = BL_{in}(x) - BL\_Ds_{in}(x)$
%\STATE $DL_{in}(x) = DL_{in}(x) - DL\_Ds_{in}(x)$
%\STATE Enqueue x
%\STATE Enqueue $BL\_Ds_{in}(x)$
%\STATE Enqueue $DL\_Ds_{in}(x)$
%\ENDIF
%\ENDFOR
%\ENDFOR
%\ENDWHILE
%\ENDIF
%
%
%\end{algorithmic}
%\end{algorithm}





\subsection{Edge Deletion}
 The update for edge deletion is also a \bfs based process. For the early termination of the \bfs, we need to determine the label-unaffected nodes in the \bfs flooding area. \bl label for example, the construction of \bl label spread the source nodes's hash value in \bfs manner, in other words, for any nodes u belong to \emph{Pre(v)}, all the hash value passed to $BL_{in}(u)$ will also be passed to $BL_{in}(v)$, symmetrically, for any nodes v belong to \emph{Suc(u)}, all the hash value passed to $BL_{out}(v)$ will also be passed to $BL_{out}(u)$. Is means for any node in the graph, its $BL_{in}$ is a union of its predecessor's $BL_{in}$, its $BL_{out}$ is a union of its successor's $BL_{out}$. Obviously, when we delete an edge (u,v) from the graph, the $BL_{in}(v)$ and $BL_{out}(u)$ will not always altered. If $BL_{in}(v)$($BL_{out}(u)$) keep unchanged, all the successors of node v's $BL_{in}$ (predecessors of node u $BL_{out}$) will not changed. Our \bfs update process will be terminated.


 When we delete an edge (u,v), we will update v and its descendent's $BL_{in}$ label in forward direction. In order to keep a record of the element that will be exclude from label, we will compute a set $BL\_Ds_{in}(v)$ which contains all the element that only be passed from u to v in label construction. It means that the elements in $BL\_Ds_{in}(v)$ are only appeared in $BL_{in}(u)$ than v's other predecessor's $BL_{in}$ label and the edge deletion will exclude all the element in the set from the $BL_{in}(v)$. Obviously, the element elimination in the $BL_{in}(v)$ will influence the $BL_{in}$ label of node v's successor but the excluded set $BL\_Ds_{in}(v)$ is not necessarily eliminate from v's successor's $BL_{in}$ label because the element in the $BL\_Ds_{in}(v)$ will not always uniquely passed throw node v. Again, for the label-affected node in v's \bfs area, we need to check the $BL\_Ds_{in}$ set for their own. \bfs process will be pruned when node's $BL\_Ds_{in}$ set is empty which means no element will be excluded from the $BL_{in}$ label and the influence of the edge deletion will not pass on. The computation of $BL\_Ds_{in}$ base on set dserence operation.


%Due to the pruned construction process, the label containment condition is not satisfied for \dl label, but but we will prove the correctness of the early termination of \dl label update latter.


xxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxx\newline
To do: use a example to explain the correctness of \dl's early termination in update\newline
xxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxx


The maintaining of \dl label in edge deletion is almost the same except that it is only needed to update the label in either forward or backward direction.
We will update \dl label in forward direction($DL_{in}$ label) and use $DL\_Ds_{in}$ to denote the excluded element set similar to $BL\_Ds_{in}$.



We discuss the edge deletion method in forward direction in algorithm 5. The backward direction computation is exactly the same except that we don't need to update \dl label anymore. We omit the backward direction algorithm from algorithm 5. At first we will initialize the $BL\_Ds_{in}(v)$ set and $DL\_Ds_{in}(v)$ set in line 1 and compute the $BL\_Ds_{in}(v)$($DL\_Ds_{in}(v)$) in line 3-4. If one of the set is not empty, it means the node v is affected by the edge deletion. We will do \bfs from node v to handle label update of all the affected nodes. In line 7-8 we update the label of node v and then node v and the updated set will be enqueued in line 10-12. Line 13 to 33 is the pruned \bfs process, each visited node will compute its $Ds_{in}$ label and check whether the set is empty. If the set is not empty, the node will be enqueued.






==> secs/experiment.tex <==
\section{Experimental Evaluation}\label{sec:exp}
In this section we will evaluate our solution against the state of the art. We implement our approach in C++, and we adopt the C++ implementations of all competitors provided by their authors. Our experiments are conducted on a machine with an Inter Xeon CPU 2.4GHz and 256GB RAM, running Centos 3.10. In our experiment we will omit the result of the method if the method require more than 24 hours or exceed our RAM to compute.


\begin{table}[h]
\caption{Real Datasets}
\begin{tabular}{cccc}
\hline
Dataset & $|V|$ & $|E|$ & $d_{avg}$ \\
\hline
LJ-DAG& 971,232&1,024,140&1.054\\
LJ& 4,847,571&68,993,773&14.23\\
Web-DAG& 371,764& 517,805&1.392\\
Web&875,713&5,105,039&5.83\\
Email-DAG&231,000 &223,004&0.965\\
Email&265,214&420,045&1.58\\
Wiki-DAG&2,281,879& 2,311,570&1.013\\
Wiki&2,394,385&5,021,410&2.09\\
Patent-DAG&3,774,768&16,518,947&4.376\\
Patent&3,774,768&16,518,947&4.376\\
Pokec-DAG& 325,892 & 379,628 &1.165\\
Pokec& 1,632,803 & 30,622,564 &18.75\\
\hline
\end{tabular}
\end{table}


Table 1 shows the datasets that we used in our experiment. As all the existing work can't work on common graph. We condense all the graph to \dagg and the graph will be added with a "\dagg" in name. All the graphs we use are directed graph. The top 6 graph are real world graph from SNAP\cite{snapnets}. LJ is social network soc-LiveJournal1. Pokec is social network soc-Pokec. They are power-law graph that have a large \scc in the graph. Web is a web graph web-Google. Wiki is a Wikipedia communication network wiki-Talk. Email is a email communication network email-EuAll. Patent is a patent citation network cit-Patents which is a \dagg. All the 6 graphs are widely used in previous work\cite{wei2018reachability,su2017reachability,zhu2014reachability}.


 In theory, our method is a common method that could handle all the graph, but actually, our method will get a performance degrade when all the graph collapse to \dagg. The reason is that the connectivity of the \dagg graph will decrease dramatically. Usually, the hub node with high connectivity have larger probability to be contained in \scc and the condense of the \scc may eliminate the hub node from our \dl label and our \dl label will lose its efficiency. However, our method is not target on \dagg graph, our method aims to eliminate the \dagg maintaining process in dynamic graph and get a better performance in update process.




\begin{table}[h]
\caption{Query Time on Real Datasets}
\begin{tabular}{ccccc}
\hline
Dataset & TOL & IP & BFL & MY \\
\hline
LJ& 46.55&-&73.02&108.64\\
Web& 40.63& 18.785&114.25&175.64\\
Email&26.80 &21.57&45.31&36.38\\
Wiki&74.89& 27.87&37.44&325.56\\
Patent&194.64&2354.76&271.87&9076\\
Pokec& 27.19 & 47.01 &80.85&58.75\\
\hline
\end{tabular}
\end{table}



Table 2 shows the result of the query experiment in millisecond. For the existing work, we compute 1 million query in \dagg graph and our method will perform on the uncondensed graph. This is because their method can't work on common graph and it will be unfair for our method to be compared on \dagg graph as we have mentioned in previous section. We compare our method with the state-of-the-art. All the method use single thread. We set both the \dl label size and the \bl label size 64. It could be seen from the graph that our method could get a comparable speed in LJ / Email and Poket. For Patent and Wiki, our method will get a dramatically performance degrade. The main reason is that Patent is a natural\dagg graph with little effective hub vertices. Our \dl label will perform badly. Although Wiki is not a \dagg, our \dl label in Wiki also badly performed. For IP method in LJ, we can't generate it's index in 24 hour, so we have no result about it query speed.

It need to be noted that for some graph with large \scc, the condense operation will transfer the graph to a much smaller graph. For LJ and Pokec, the largest \scc contains about 80 percent of the nodes and 95 percent of the edges. The condensed graph will be more than tens times smaller than the uncondensed graph. As our method works on the uncondensed graph, the \bfs process will be heavy burdened compared to the condensed graph.


\subsection{Parameters in DBL}
We study how the parameters used in DBL affect the performance of DBL. There are two indexes that we used in our method. Both \dl and \bl will generate label in bit vector manner. The length of the \dl label depends on the number of the hub nodes that we used in \dl. It seems that the more hub nodes we use the better performance we will get in query, but in fact the \dl index size will expand linearly and the query performance will degrade as longer label will need more time to compute set intersection. Therefor, a reasonable \dl label size is needed. Similarly, \bl label store the reachability information in hash vector. There will be false positive answer in the hash vector containment computation which will affect our query performance. If we set a larger \bl label the false positive rate will decrease. Same with \dl index, the expand of \bl label will also increase the index size in linear speed.


 We show the query time that depends on the size of the label in figure xxxxxxxxx. We use LJ as an example. Figure 1a and 1b shows the query time with different label size. We will set \bl label size 64 in default in figure 1a and set \dl label size 64 in figure 1b.


In fact, the optimised size of \bl/\dl label is graph depends. It depends on the connectivity and number of hub nodes. We will set the default \dl/\bl label size 64 in our experiment as it shows reasonable space efficiency and query speed.

\subsection{Update in DBL}
The most challenging work in dynamic graph reachability query is that we need to control the update overhead in an acceptable level. Obviously, the update time should be much less than the re-construction of the index. Otherwise, we could reconstruct the index after insertion/deletion of edges. 



We will show our experiment for index update in this section. We compare our method against TOL and IP as they are the state-of-the-art method in dynamic graph reachability query method.

Table 3 shows the total time for 1000 edges insertion in seconds. It can be seen from the table that our method could get a better performance for tens to hundred times.

Table 4 is the total deletion time for 1000 edges in seconds. Again, our method could get a much better performance. The main reason is that our approach could get an early termination in \bfs update process. Both the \bl label and \dl label will stop update process when the \bfs visited label will not be affected. In fact, both our \bl and \dl label will be set 64 bit in default, which is a rather small label size for graph with million nodes. For \bl lable, more than ten thousands nodes will be hashed to the same bit. This means there are thousands of "alternatives" in update process for the same bit. It is very easy for a bit in a label to be filled.

\begin{table}[h]
\caption{Edge Insertion Time on Real Datasets}
\begin{tabular}{cccc}
\hline
Dataset & TOL & IP & MY \\
\hline
LJ&0.32&1190&0.003\\
Web&1.14&-&0.703\\
Email&0.05&9.24&0.016\\
Wiki&0.43&12.3&0.004\\
Patent&5.46&-&0.139\\
Pokec&48.05&-&0.006\\
\hline
\end{tabular}
\end{table}


 \begin{table}[h]
\caption{Edge Deletion Time on Real Datasets}
\begin{tabular}{cccc}
\hline
Dataset & TOL & IP & MY \\
\hline
LJ&50.45&4.53&0.55\\
Web&18.74&0.87&0.12\\
Email&9.91 &0.32&0.054\\
Wiki&187.71&12.3&0.36\\
Patent&103.35&-&0.69\\
Pokec&64.59&0.9&0.192\\
\hline
\end{tabular}
\end{table}


\subsection{Scalability with Threads}







\subsection{Parallel Query}
We parallel our query approach with openMP and CUDA. We show the total time for 1 million query in table. For openMP implementation we use Inter Xeon CPU 2.4GHz with 10 cores. For CUDA implementation, we use Tesla p100 with 12GB memory.Due to the pruned process in \bfs, only a few nodes will be visited in each layer, so we will use a block with a warp to process a \bfs. We will parallel 1024 \bfs with 1024 block.




\begin{table}[h]
\caption{Query Time in Parallel}
\begin{tabular}{cccc}
\hline
Dataset & Single Thread & openMP & CUDA \\
\hline
LJ&108.64&16.42&4.06\\
Web&175.64&12.36&6.18\\
Email&36.38 &4.07&2.77\\
Wiki&325.56&26.67&6.89\\
Patent&9076&460&345\\
Pokec&58.75&8.96&3.05\\
\hline
\end{tabular}
\end{table}




==> secs/label.tex <==
\begin{algorithm}[t]
	\caption{label update for edge insertion}
	\begin{algorithmic}[1]
		\Require
		Graph $G(V,E)$, \dl label, Inserted edge $(u,v)$
		\Ensure
		Updated \dl label
		\If{ $\dl_{out}(u) \cap \dl_{in}(v) == \emptyset$ }
		\State Initialize an empty queue and enqueue $v$\label{algo:bfs-start}
		\While{queue is not empty}
		\State $p \gets $ pop queue
		\For{vertex $ x \in Suc(p)$}
		\If{ $\dl_{in}(u) \not\subseteq  \dl_{in}(x)$ or $\bl_{in}(u) \not\subseteq  \bl_{in}(x)$ }
		\State $\dl_{in}(x) \gets \dl_{in}(x) \cup \dl_{in}(u)$
        \State $\bl_{in}(x) \gets \bl_{in}(x) \cup \bl_{in}(u)$
		\State enqueue x
		\EndIf
		\EndFor
		\EndWhile
		\EndIf
        \State  //Update $\dl_{out}$ and $\bl_{out}$ in the reverse direction, which is symmetrical to the update of $\dl_{in}$ and $\bl_{in}$.
	\end{algorithmic}
	\label{algo:insert}
\end{algorithm}

\section{\dl and \bl Maintenance}\label{sec:lan}

For both \dl and \bl index, we treat a vertex update operation as a set of edge update operations.
When inserting a new vertex, we create \dl and \bl labels followed by inserting all the related edges by the corresponding edge insertion algorithms. Likewise, for vertex deletion, we remove all its edges that are connected to the vertex and invoke the corresponding edge deletion algorithms.
Thereby, we focus on presenting the edge insertion and deletion algorithms in the remaining sections of this paper.
%We present the edge insertions and deletions in Section~\ref{sec:lan:insert} and~\ref{sec:lan:delete}, respectively.
%We focus on the edge update in this section and vertex updates are discussed in Section~\ref{sec:discussion}.
%We focus on edge insertion/deletion in this section and vertex updates are discussed in Section~\ref{sec:discussion}.






\begin{figure*}[t]
	\subfigure[Insert edge $(v_9,v_2)$ ]{
	\begin{minipage}{0.45\columnwidth}
		\label{fig:example4}
		\includegraphics[width=3.7cm]{example/example4.eps}
	\end{minipage}
	}
	\hfill
	\subfigure[$\dl_{in}$ label update]{
	\begin{minipage}{0.45\columnwidth}
%	\small
		\centering
		\begin{tabular}{||c|c||}
			\hline
			\rowcolor[gray]{.9}	
			\hline
			$v$	    &	$\dl_{in}$		                                    \\ \hline
			$v_1$	&	$\emptyset	\rightarrow	\emptyset$	                \\ \hline
			$v_2$	&	\textcolor{red}{$\emptyset	\rightarrow	\{v_5\}$}		\\ \hline
			$v_3$	&	$\emptyset	\rightarrow	\emptyset$                 \\ \hline
			$v_4$	&	$\emptyset	\rightarrow	\emptyset$	                \\ \hline
			$v_5$	&	$\{v_5\}		\rightarrow \{v_5\}$	                    \\ \hline
			$v_6$	&	$\{v_5\}		\rightarrow	\{v_5\}$	                    \\ \hline
			$v_7$	&	$\emptyset	\rightarrow	\emptyset$	                \\ \hline
			$v_8$	&	$\{v_5,v_8\}	\rightarrow		\{v_5,v_8\}$		        \\ \hline
			$v_9$	&	$\{v_5\}		\rightarrow		\{v_5\}$	                \\ \hline
			$v_{10}$	&	$\{v_5,v_8\}	\rightarrow	\{v_5,v_8\}$	        	\\ \hline
			$v_{11}$	&	$\{v_5\}		\rightarrow	\{v_5\}$		            \\ \hline
		\end{tabular}
		\label{fig:dl-label-insert}
	\end{minipage}
	}
    \hfill
    \subfigure[$\bl_{in}$ label update]{
	\begin{minipage}{0.45\columnwidth}
%	\small
		\centering
		\begin{tabular}{||c|c||}
			\hline
			\rowcolor[gray]{.9}	
			\hline
			$v$	    &	$\bl_{in}$		                                                       \\ \hline
			$v_1$	&	$\{0\}	\rightarrow	\{0\}$	                                           \\ \hline
			$v_2$	&	\textcolor{red}{$\{1\}	\rightarrow	\{0,1\}$}		                   \\ \hline
			$v_3$	&	$\{1\}	\rightarrow	\{1\}$                                                \\ \hline
			$v_4$	&	$\{0\}	\rightarrow	\{0\}$	                                           \\ \hline
			$v_5$	&	\textcolor{red}{$\{1\}		\rightarrow \{0,1\}$}	                    \\ \hline
			$v_6$	&	\textcolor{red}{$\{1\}		\rightarrow	\{0,1\}$}	                    \\ \hline
			$v_7$	&	$\{1\}	\rightarrow	\{1\}$	                                    \\ \hline
			$v_8$	&	$\{0,1\}	\rightarrow	\{0,1\}$		                                  \\ \hline
			$v_9$	&	$\{1\}	\rightarrow		\{1\}$	                                  \\ \hline
			$v_{10}$	&	$\{0,1\}	\rightarrow	\{0,1\}$	        	                   \\ \hline
			$v_{11}$	&	$\{1\}		\rightarrow	\{1\}$		                          \\ \hline
		\end{tabular}
		\label{fig:bl-label-insert}
	\end{minipage}
	}
	\caption{label update for inserting edge $(v_9,v_2)$}
	\label{fig:insert}
\end{figure*}







\subsection{Label Update for Edge Insertions}\label{sec:lan:insert}
When inserting a new edge $(u,v)$,
all vertices in $Anc(u)$ can reach all vertices in $Des(v)$.
On a high level, all nodes that could reach $u$ should also reach vertices in $Des(v)$. In other words, all the nodes that could be reached by $v$ should also be reached by vertices in $Anc(u)$.
Thus, we should maintain the $\dl$ label like this:
1) update the label by adding $\dl_{in}(u)$ into $\dl_{in}(x)$ for all $x \in Des(v)$; and
2) adding $\dl_{out}(v)$ into $\dl_{out}(x)$ for all $x \in Anc(u)$.
Similarly, the $\bl$ label should be handle in the same way.


Algorithm~\ref{algo:insert} depicts the $\bl_{in}$ and $\dl_{in}$ label update process. We test whether the newly inserted edge adds extra connectivity to the graph in Line 1.
If \dl label can determine that vertex $v$ is reachable by vertex $u$ in the original graph before the edge insertion, the insertion will not trigger any label update.
%\textcolor{blue}{It's need to mention that, as \dl is a partial cover label, there is a possibility that vertex $u$ could reach vertex $v$, but the label intersection is a null set. In this scenario, the update will make up the originally omitted reachability information.}
Lines~\ref{algo:bfs-start}-\ref{algo:bfs-end} describe a \bfs process with pruning. For a visited vertex $x$, we prune $x$ without traversing $Des(x)$ when all the vertices's label in $Des(x)$ are deemed to be unaffected.



\begin{example}
Figure~\ref{fig:insert} shows an example of label update for an edge insertion. $\dl_{in}$ and $\bl_{in}$ labels are presented with brackets. Give an edge $(v_9,v_2)$ inserted, $\dl_{in}(v_9)$ and is copied to $\dl_{in}(v_2)$, similarly, $\bl_{in}(v_9)$ is copied to $\bl_{in}(v_2)$. Then an inspection will be processed on nodes $v_{5}$ and $v_{6}$. Since $\dl_{in}(v_9)$ is a subset of $\dl_{in}(v_5)$ and $\dl_{in}(v_6)$, only $\bl_{in}(v_5)$ and $\bl_{in}(v_6)$ will be updated. Then, we will inspect $v_8$ and $v_9$. The update progress is terminated as no nodes will be updated and enqueued.

\end{example}





\subsection{Label Update for Edge Deletions}\label{sec:lan:delete}
Deleting an edge is more complicated than inserting an edge. When an edge $(u,v)$ is deleted, not all the connectivities between $Anc(u)$ and $Des(v)$ are affected. The status of a vertex pair's reachability changes if and only if the paths connecting them always include the deleted edge. Thus, we need to carefully adjust the label so that only the reachability information carried by the deleted edge is removed.


Our deletion algorithm is based on an important observation that if a vertex $u$ is not a landmark, $\dl$ and $\bl$ label satisfy the following equation:

\begin{equation}
\begin{split}
  \dl_{in}(u)=\bigcup_{p\in{Pre(u)}}\dl_{in}(p) \\
  \dl_{out}(u)=\bigcup_{q\in{Suc(u)}}\dl_{out}(q) \\
  \bl_{in}(u)=\bigcup_{p\in{Pre(u)}}\bl_{in}(p) \\
  \bl_{out}(u)=\bigcup_{q\in{Suc(u)}}\bl_{out}(q)
\end{split}
\end{equation}



In other words, all the elements in $\dl_{in}(u)$($\bl_{in}(u)$) are propagated from vertices in $Pre(u)$ and all the elements in $\dl_{out}(u)$($\bl_{out}(u)$) label are propagated from vertices in $Suc(u)$. This is because when we insert new edges, the label is propagated in a \bfs manner (Algorithm~\ref{algo:insert}). If vertex $x$ is visited in edge insertion, all the vertices belonging to $Des(x)$ are visited. As a result, $\dl_{in}$($\bl_{in}$) label of the vertices belong to $Des(x)$ is a superset of $\dl_{in}(x)$($\bl_{in}(x)$). Similarly, $\dl_{out}$($\bl_{out}$) labels of all vertices in $Anc(x)$ are supersets of $\dl_{out}(x)$($\bl_{out}(x)$).




To properly update the label, we need to make sure that the labels which are propagated through the deleted edge only (during index maintenance) will be excluded from the affected vertices. For deleted edge $(u,v)$, take $\dl_{in}$ label as example, if there exist labels that are propagated through $(u,v)$ only, we need to update the vertices that belong to $Des(v)$. Hence, all the vertices in $Des(v)$ need to check $\dl_{in}$ label propagated by their predecessors. $\dl_{out}$ label for the vertices in $Anc(u)$ is handled in a similar manner. In summary, all the vertices belong to $Des(v)$ need to check their predecessors' $\dl_{in}$ label to make sure the edge deletion has been reflected in the label. Symmetrically, the vertices belong to $Anc(u)$ check their successors' $\dl_{out}$ label to guarantee the consistency.


\begin{figure*}[t]
	\subfigure[Delete edge $(v_6,v_9)$ ]{
	\begin{minipage}{0.45\columnwidth}
		\label{fig:example5}
		\includegraphics[width=3.6cm,height=5.3cm]{example/example5.eps}
	\end{minipage}
	}
	\hfill
	\subfigure[$\dl_{in}$ label update]{
	\begin{minipage}{0.45\columnwidth}
%	\small
		\centering
		\begin{tabular}{||c|c||}
			\hline
			\rowcolor[gray]{.9}	
			\hline
			$v$ 	&	$ \dl_{in}$		        \\ \hline
			$v_1$	&	$\emptyset	\rightarrow	\emptyset$			\\ \hline
			$v_2$	&	$\emptyset	\rightarrow	\emptyset$		\\ \hline
			$v_3$	&	$\emptyset \rightarrow	\emptyset$		\\ \hline
			$v_4$	&	$\emptyset	\rightarrow	\emptyset$			\\ \hline
			$v_5$	&	$\{v_5\}		\rightarrow	\{v_5$\}	\\ \hline
			$v_6$	&	$\{v_5\}		\rightarrow	\{v_5$\}	\\ \hline
			$v_7$	&	$\emptyset	\rightarrow	\emptyset$		\\ \hline
			$v_8$	&	$\{v_5,v_8\}	\rightarrow		\{v_5,v_8$\}		\\ \hline
			$v_9$	&	\textcolor{red}{$\{v_5\}		\rightarrow		\emptyset$}	\\ \hline
			$v_{10}$	&	$\{v_5,v_8\}	\rightarrow	\{v_5,v_8\}$		\\ \hline
			$v_{11}$	&	\textcolor{red}{$\{v_5\}		\rightarrow	\emptyset$}	\\ \hline
		\end{tabular}
		\label{fig:dl-label-delete}
	\end{minipage}
	}
    \hfill
    \subfigure[$\bl_{in}$ label update]{
	\begin{minipage}{0.45\columnwidth}
%	\small
		\centering
		\begin{tabular}{||c|c||}
			\hline
			\rowcolor[gray]{.9}	
			\hline
			$v$	    &	$\bl_{in}$		                                                       \\ \hline
			$v_1$	&	$\{0\}	\rightarrow	\{0\}$	                                           \\ \hline
			$v_2$	&	$\{1\}	\rightarrow	\{1\}$		                   \\ \hline
			$v_3$	&	$\{1\}	\rightarrow	\{1\}$                                                \\ \hline
			$v_4$	&	$\{0\}	\rightarrow	\{0\}$	                                           \\ \hline
			$v_5$	&	$\{1\}		\rightarrow \{1\}$	                    \\ \hline
			$v_6$	&	$\{1\}		\rightarrow	\{1\}$	                    \\ \hline
			$v_7$	&	$\{1\}	\rightarrow	\{1\}$	                                    \\ \hline
			$v_8$	&	$\{0,1\}	\rightarrow	\{0,1\}$		                                  \\ \hline
			$v_9$	&	\textcolor{red}{$\{1\}	\rightarrow		\emptyset$}	                                  \\ \hline
			$v_{10}$	&	$\{0,1\}	\rightarrow	\{0,1\}$	        	                   \\ \hline
			$v_{11}$	&	$\{1\}		\rightarrow	\{1\}$		                          \\ \hline
		\end{tabular}
		\label{fig:bl-label-insert}
	\end{minipage}
	}
	\caption{$\dl$ label update for deleting edge $(v_6,v_9)$. $\dl_{out}$ update are omitted.}
	\label{exp:delete}
	\vspace{-1em}
\end{figure*}





For the sake of simplification, we only depict the \dl label update process for edge deletions in Algorithm \ref{algo:delete}, the update of \bl label is totally the same thus omitted in the paper.
We initialize a set $R_{in}(v)$ (Line 1), which keeps the elements that should be excluded from $\dl_{in}(v)$.
$R_{in}(v)$ is computed by taking the difference between $\dl_{in}(v)$ with $\dl_{in}$ labels of $v$'s predecessor (Lines 3-4).
Subsequently, we check whether vertex $v$ is a landmark in Lines 5-6, because a landmark always keeps its itself as a label element in both $\dl_{in}$ and $\dl_{out}$. If $R_{in}(v)$ is an empty set, it means no label element is excluded from $\dl_{in}(v)$ and the edge $(u,v)$ does not uniquely carry the reachability information. Hence all the vertices in $Des(v)$ are unaffected and the update process is terminated.
If the $R_{in}(v)$ set is not empty, the \bfs process is executed to inspect vertices in $Des(v)$ (Lines 9-20).
%Lines 9-20 show the \bfs procedure.
%A \bfs queue is initialized in line 9 which keep the \bfs visited node and its corresponding $R_{in}$ set.

For vertex $p$ visited by the \bfs, we inspect all $\dl_{in}$ labels of the vertices belong to $Suc(p)$ (Lines 12-20), compute $R_{in}$ by set difference operations from Lines 14-15 and check if the vertex is a landmark (Lines 16-17). If the $R_{in}$ set is not empty (Lines 18-20), the vertex is enqueued as its descendant's label may be altered by the edge deletion. We also need to update $\dl_{out}$ in the reverse direction from $u$.
Since it is symmetrical to the update of $\dl_{in}$, we omit the pseudo code.




%\begin{figure}[t]
%	\centering \subfigure{\includegraphics[width=0.45\columnwidth]{example/example5.eps}}
%	\caption{\dl label update for deleting edge $(6,9)$}
%	\label{fig:example5}
%\end{figure}




\begin{example}
Figure~\ref{exp:delete} shows an example of \dl label update after an edge deletion. If edge $(v_6,v_9)$ is deleted from the graph, the label element "$v_5$" in $\dl_{in}(v_9)$ is only passed from vertex $v_6$ as vertex $v_6$ is the only predecessor of vertex $v_9$. Therefore, "$v_5$" is included in $R_{in}(v_9)$ and excluded from $\dl_{in}(v_9)$. After the update of $\dl_{in}(v_9)$, the \bfs process inspects the successors of vertex $v_9$. When vertex $v_{11}$ is visited, it finds that label element "$v_5$" is be passed from edge $(v_7,v_{11})$. As a result, "$v_5$" is excluded from $\dl_{in}(v_{11})$. Henceforth, vertex $v_5$ is inspected. Since vertex $v_5$ is a landmark, $R_{in}(v_5)$ excludes $v_5$ and become an empty set. Vertex $v_5$ will not be enqueued and the update process is terminated. Similarly, only $\bl_{in}(v_9)$ will be affected in this example. We omit the update of $\dl_{out}$ and $\bl_{out}$ in this example.
\end{example}




\begin{algorithm}[t!]
	\caption{\dl Label update for edge deletion}
	\begin{algorithmic}[1]
		\Require
		Graph $G(V,E)$, \dl label, Deleted edge $(u,v)$
		\Ensure
		Updated \dl label
		
		\State // Update $\dl_{in}$ in the forward direction
		\State Initialize $R_{in}(v) \gets \dl_{in}(u)$ \label{algo:dl:delete-start}
		\ForAll{p in \emph{Pre(v)}}
		\State $R_{in}(v) = R_{in}(v) - \dl_{in}(p)$
		\EndFor
		\If{$v$ is landmark vertex}
		\State $R_{in}(v) = R_{in}(v) - v$
		\EndIf
		
		\If{$R_{in}(v) \neq \emptyset$}
		\State $\dl_{in}(v) = \dl_{in}(v) - R_{in}(v)$
		\State Initialize an empty queue and enqueue $(v,R_{in}(v))$
		\While{queue is not empty}
		\State $(p,R_{in}(p)) \gets $ pop queue
		\For{node x in \emph{Suc(p)}}
		\State $R_{in}(x) = R_{in}(p)$
		\For{node y in \emph{Pre(x)}}
		\State $R_{in}(x) = R_{in}(x) - \dl_{in}(y)$
		\EndFor
		\If{$x$ is landmark vertex}
		\State $R_{in}(x) = R_{in}(x) - x$
		\EndIf
		\If{$R_{in}(x) \neq \emptyset$}
		\State $\dl_{in}(x) = \dl_{in}(x) - R_{in}(x)$
		\State enqueue $(x,R_{in}(x))$ \label{algo:dl:delete-end}
		\EndIf
		\EndFor
		\EndWhile
		\EndIf
		
		\State // Update $\dl_{out}$ in the reverse direction, which is symmetrical to the update of $\dl_{in}$ (Lines~\ref{algo:dl:delete-start}-\ref{algo:dl:delete-end}).
		%		\State //Update $\dl_{in}$ label in forward direction
		%	    \State Initialize $R_{out}(u) \gets \dl_{out}(v)$
		%		\ForAll{q in \emph{Suc(u)}}
		%		\State $R_{out}(u) = R_{out}(u) - \dl_{out}(q)$
		%		\EndFor
		%		\If{u is landmark vertex}
		%		\State $R_{out}(u) = R_{out}(u) - u$
		%		\EndIf
		%		\If{$R_{out}(u) \neq \emptyset$}
		%		\State $\dl_{out}(u) = \dl_{out}(u) - R_{out}(u)$
		%		\State Initialize an empty queue and enqueue $(u,R_{out}(u))$
		%		\While{queue is not empty}
		%		\State $(q,R_{out}(q)) \gets $ pop queue
		%		\For{node $x$ in Pre(q)}
		%		\State $R_{out}(x) = R_{out}(q)$
		%		\For{node y in \emph{Suc(x)}}
		%		\State $R_{out}(x) = R_{out}(x) - \dl_{out}(y)$
		%		\EndFor
		%		\If{$x$ is landmark vertex}
		%		\State $R_{out}(x) = R_{out}(x) - x$
		%		\EndIf
		%		\If{$R_{out}(x) \neq \emptyset$}
		%		\State $\dl_{out}(x) = \dl_{out}(x) - R_{out}(x)$
		%		\State enqueue $(x,R_{out}(x))$
		%		\EndIf
		%		\EndFor
		%		\EndWhile
		%		\EndIf
	\end{algorithmic}
	\label{algo:delete}
\end{algorithm}


%Note that we only present the insertion and deletion algorithms for \dl label in this section. To build \dl for scratch, we can repeatedly call the insertion algorithm for each edge in the graph or invoke a batch construction algorithm which can be much more efficient. Nevertheless, we focus on discussing the update algorithms and leave the batch construction algorithm in the appendix for interested readers.






%Algorithm 4 shows the query method that performed by \dl label. Same with 2-Hop label, the query will answer true when there are some intermediate node in their label(line 1-4). If the label can't give a positive answer, we are not sure whether $v$ is reachable by $u$ as our \dl label just partially cover the reachability information. A pruned \bfs will be run to make sure their reachability. For visited vertex w, it will be enqueued $iff$ $DL_{out}(u) \cap DL_{in}(w) = \emptyset$, if w is conducted reachable by u, then all the vertices belong to $Des(w)$ should be judged reachable by u as we have mentioned their $DL_{in}$ are superset of $DL_{in}(w)$. Because $v$ has been tested unreachable by \dl label, the vetex w and its descendants should be pruned from the \bfs if w is judged reachable by u by \dl label. Line 6-16 shows the pruned \bfs process.


%\begin{algorithm}[ht]
%\caption{\dl Query}
%\begin{algorithmic}[1]
%\REQUIRE
%Graph G(V,E), \dl Index, Query:$q(u,v)$
%\ENSURE
%Result of the query
%\IF{$DL_{out}(u) \cap DL_{in}(v)$ }
%\STATE Set result = true
%\STATE Break
%\ENDIF
%\STATE //Do \bfs from u in G(V,E)
%\WHILE{\bfs queue is not empty}
%\FOR{w that \bfs visited}
%\IF{$w = v$}
%\STATE Set $result=true$
%\STATE Break
%\ENDIF
%\IF{$DL_{out}(u) \cap DL_{in}(w) = \emptyset$}
%\STATE Enqueue w
%\ENDIF
%\ENDFOR
%\ENDWHILE
%\end{algorithmic}
%\end{algorithm}





%\begin{example}
%If delete edge $(6,9)$ from the graph, as vertex 6 is the only predecessor of vertex 9, label node 5 will be excluded from $\dl_{in}(9)$, after the update of $\dl_{in}(9)$, \bfs process will inspect the successors of vertex 9,
%\end{example}


%\begin{example}
%If query $q(2,11)$, because there is an intermediate node 5 in $DL_{out}(2)$ and $DL_{in}(11)$, it could answer true directly by label. if query $q(9,7)$, because %$DL_{out}(9) \cap DL_{in}(7) = \emptyset$, it can't give answer by label, vertex 9 will be enqueued for \bfs, as vertex 5 and 11 are judged reachable by 9 by \dl %label, they will not enqueue for \bfs, as a result, the \bfs process is terminated. \dl will answer false to the query $q(9,7)$.
%\end{example}




%Ideally, we want to get a minimum set of nodes that could cover as much reachable information as we can in the graph. But actually, the completely computation to select the best cover set is not practical for large graph as it have been proved in \cite{cohen2003reachability} that the computation is NP-hard. So we use a heuristic method to select the cover set. We compute the product of all the vertices's in-degree and out-degree and use the product to sort the vertices in an descending order. We select the top N nodes as the hub vertices to construct the 2-Hop index. To accelerate the computing of label intersection, we use bit vectors to contain all the labels, in this way the label size will decrease dramatically and we could also get a faster intersection speed.

%We show the algorithm to construct the \dl index in Algorithm 1. The algorithm will output the Dynamic Landmark Index. Every node in the graph will include the $DL_{in}$ and $DL_{out}$. Node v's $DL_{in}(v)$ will include all the hub nodes that could reach v and $DL_{out}(v)$ will include all the hub nodes that could be reached by v. At first we will compute the product M(v) (line 2-4) as we aforementioned and sort all the nodes (line 5). Then we select the top L nodes as the hub node where L is a user predefined variable that determine how many hub nodes we use in our algorithm. For every hub node that we select we will do pruned \bfs in bi-direction (line 6-23) that is to do \bfs in the graph G(V,E) and it's reversed graph G'(V,E') respectively. In each \bfs with the source hub node v, only the nodes that are determined unreachable by the \dl label will enqueue and the corresponding bit(equal to the source node's serial number) of the label will be set to 1 (line 9-14,line 18-23) which means the node could be reached by v(or v is reachable by the node). The pruned operation will reduce the elements in the label and significantly accelerate the \bfs.


==> secs/literature.tex <==
\section{Related Works}\label{sec:lit}

==> secs/preliminary.tex <==
\section{Preliminaries}\label{sec:pre}
A directed graph is modeled as G=(V,E), V is the vertex set and E is the edge set. The reversed graph is modeled as G'=(V,E') which means that all the edges are in opposite direction. The number of vertices in G is denoted as $n=|V|$ and the number of edges in G is denoted as $m=|E|$. We define a path from vertex u to vertex v as \emph{path(u,v)}=(u,$w_1$,$w_2$,$w_3$...,v) where $w_i$ is vertex in V and all the path vertex are connected in path order by edges in E. Vertex v is reachable by u iff there exist a \emph{path(u,v)}. For two vertices u and v in V, if there exist an edge from u to v, we denote the edge as (u,v). In addition, we use \emph{Suc(u)} to denote the direct successors of node u, respectively, the direct predecessor of u is denoted as \emph{Pre(u)}. Similarly, we denote all the ancestor of node u as \emph{Anc(u)} and all the descendent of vertex u as \emph{Des(u)}.


==> secs/reachability_query.tex <==
\section{Reachability Query}\label{sec:rq}

There are two motivations that we propose DBL. Firstly, \dagg maintaining process is really time consuming in dynamic graph, we want to propose a method that could directly works on primitive graph that could avoid \dagg maintaining process. Secondly, all the existing Lable+G method are efficient in answer negative query on sparse graph but the label pruned power which is the ratio of the queries that could be directly answered by label will degrade as the graph's average degree increase\cite{su2017reachability}. The degeneration of the label pruned efficiency will dramatically lower the query speed.

We proposed DBL as our solution. For the first motivation, we need a method that is \dagg free which means that our method should be capable of handle graphs with cycle and huge \scc. So the \dfs based method and topological order based method are unacceptable. For the second motivation, We want to construct a balance label group which means that there may be several different labels in our method that could be complementary to each other, so they could handle most of the graph no matter it is a sparse graph or dense graph. As a consequence, we make a combination of \dl and \bl. \bl is a variant of BFL\cite{su2017reachability} which have been proved to be efficiency in sparse graph. Different from BFL, \bl is a \bfs based method that could works well on common graph. But it will also get a severe efficiency degeneration as the average degree increase. As a complementary to \bl, \dl is a method that could handle graph with high connectivity. It's based on an observation that as the average degree increase, the connectivity of the graph will be greatly strengthened and hub vertex will be more and more efficiency in reachable information cover. In extreme case, all the node in the graph are in a \scc in which all the reachability information could be covered by a single intermediate node label.

With the combination of \dl and \bl, our label set could get a balanced pruned power on reachability query. In sparse graph, most of the query will be negative which could be efficiently answered by \bl. As the average degree increase, the connectivity of the graph will be greatly enhanced, the efficiency of \bl label will decrease but the efficiency of \dl label will increase. The overall prune efficiency will still be hold to a acceptable level.

The complete query process in DBL include two part: label query and pruned \bfs query. Most of the queries will be answered by DBL label. A few unanswered query will be passed to pruned \bfs process. We show the query algorithm in algorithm 3. \dl label is used to cover most of the positive query(line 2-5) and \bl label cover most of the negative query(line 6-9). It is notable that \bl is bidirectional. After label query, the remaining unanswered query will be passed to \bfs query process. For every node that \bfs visited there will be a detection that whether the destination node v is visited(line 14-17). The \bfs process is a pruned by \dl label and \bl label(line 18-20). For the first enqueue condition judged by \dl label, if the \bfs visited node w could be judged reachable by u and the destination node v is an descendent of node w, then the node v must be judged reachable by u in the line 2-5. This is based on the special construction process of \dl. If node q has been judged reachable by node p by \dl label, then all the descendent nodes of node q should be judged reachable by node p by \dl label.  Similarly, the \bl pruning condition eliminate the nodes that are not the ancestor node of destination node v. Obviously, the pruning process in \bfs greatly minimize the search area and accelerate our \bfs search.




%
%\begin{algorithm}[ht]
%\caption{DBL Query}
%\begin{algorithmic}[1]
%\REQUIRE
%Graph G(V,E), Query Index, Query: if v is reachable by u
%\ENSURE
%Result of the query
%\STATE //label query
%\IF{$DL_{out}(u) \cap DL_{in}(v)$ }
%\STATE Set result = true
%\STATE Break
%\ENDIF
%\IF{$BL_{In}(u) \not\subseteq BL_{In}(v)$ \newline or $BL_{Out}(v) \not\subseteq BL_{Out}(u)$}
%\STATE Set $result=false$
%\STATE Break
%\ENDIF
%\STATE //\bfs query
%\STATE //Do \bfs from u in G(V,E)
%\WHILE{\bfs queue is not empty}
%\FOR{w that \bfs visited}
%\IF{$w = v$}
%\STATE Set $result=true$
%\STATE Break
%\ENDIF
%\IF{$DL_{out}(u) \cap DL_{in}(w) = \emptyset$ \newline and $BL_{In}(w) \subseteq BL_{In}(v)$ \newline and $BL_{Out}(v) \subseteq BL_{Out}(w)$}
%\STATE Enqueue w
%\ENDIF
%\ENDFOR
%\ENDWHILE
%\end{algorithmic}
%\end{algorithm}






